Depth-2 Neural Networks Under a Data-Poisoning Attack

In this work, we study the possibility of defending against data-poisoning attacks while training a shallow neural network in a regression setup. We focus on doing supervised learning for a class of depth-2 finite-width neural networks, which includes single-filter convolutional networks. In this class of networks, we attempt to learn the network weights in the presence of a malicious oracle doing stochastic, bounded and additive adversarial distortions on the true output during training. For the non-gradient stochastic algorithm that we construct, we prove worst-case near-optimal trade-offs among the magnitude of the adversarial attack, the weight approximation accuracy, and the confidence achieved by the proposed algorithm. As our algorithm uses mini-batching, we analyze how the mini-batch size affects convergence. We also show how to utilize the scaling of the outer layer weights to counter output-poisoning attacks depending on the probability of attack. Lastly, we give experimental evidence demonstrating how our algorithm outperforms stochastic gradient descent under different input data distributions, including instances of heavy-tailed distributions.

==> settings.tex <==


%%%%%%%% Packages %%%%%%%%%%%
\usepackage{amsmath,amssymb,amsxtra,mathtools,amsthm}
\usepackage{array}
\usepackage{graphicx}
%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage{algpseudocode}
\usepackage{dsfont}
\usepackage{bm}
%\usepackage{caption}
\usepackage{verbatim}
\usepackage{enumerate}
\usepackage{parskip}
\newcommand{\ignore}[1]{}


\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{bm}
\usepackage{dsfont}
\usepackage{enumitem}
\usepackage{mathtools}

%%%

%%% For appendix



%%%

%%% For main text

\def\ve#1{\mathchoice{\mbox{\boldmath$\displaystyle\bf#1$}}
{\mbox{\boldmath$\textstyle\bf#1$}}
{\mbox{\boldmath$\scriptstyle\bf#1$}}
{\mbox{\boldmath$\scriptscriptstyle\bf#1$}}}

\newcommand{\g}{{\ve g}}
\newcommand{\ind}[1]{\mathds{1}_{\left\{#1\right\}}}
\newcommand{\mymod}[1]{\ (\mathrm{mod}\ #1)}
\newcommand{\norm}[2][]{#1\lVert #2 #1\rVert}
\newcommand{\s}{\textrm{s}}
\newcommand{\w}{{\ve w}}
\newcommand{\x}{{\ve x}}
\newcommand{\y}{{\ve y}}
\newcommand{\z}{{\ve z}}
\newcommand{\A}{\textrm{A}}
\newcommand{\C}{\textrm{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\textrm{I}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\R}{\mathbb{R}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\relu}{{\textrm{ReLU}}}

%%%

%%% For appendix

\renewcommand{\a}{{\ve a}}
\newcommand{\q}{{\ve q}}

\newcommand{\mynote}[1]{\begin{center}
\fbox{\begin{minipage}{\columnwidth}{\begin{center} {\color{firebrick} \vspace{2mm} #1 \vspace{2mm}} \end{center}} \end{minipage}}
\end{center}}

\definecolor{firebrick}{RGB}{178,34,34}

%%%

\newtheorem{assn}{Assumption}
\newtheorem{dfn}{Definition}
\newtheorem{lm}{Lemma}
\newtheorem{rmrk}{Remark}
\newtheorem{thm}{Theorem}
%%%% Special Environments %%%%%%
\usepackage{color}
\definecolor{clemson-orange}{RGB}{234,106,32}
\definecolor{chicago-maroon}{RGB}{128,0,0}
\definecolor{cincinnati-red}{RGB}{190,0,0}
\definecolor{soft-cyan}{RGB}{68,85,90}
\definecolor{firebrick}{RGB}{178,34,34}
\definecolor{crimson}{RGB}{220,20,60}

\usepackage{hyperref}
\hypersetup{
  colorlinks   = true,    % Colours links instead of ugly boxes
  urlcolor     = blue,    % Colour for external hyperlinks
  linkcolor    = firebrick,    % Colour of internal links
  citecolor    = blue      % Colour of citations
}

% \let\bbordermatrix\bordermatrix
% \patchcmd{\bbordermatrix}{8.75}{4.75}{}{}
% \patchcmd{\bbordermatrix}{\left ( }{\left [ }{}{}
% \patchcmd{\bbordermatrix}{\right )}{\right ]}{}{}
%\setlength{\parindent}{0pt}
% \AtBeginDocument{%
% \setlength{\parskip}{1\baselineskip plus 2pt}%
% }

% \setlength{\parskip}{1\baselineskip plus 2pt}
% \usepackage[parfill]{parskip}
% \newcommand{\removed}[1]{} 

% \newtheorem{assumption}{Assumption}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{question}[theorem]{Question}
% \newtheorem{conjecture}[theorem]{Conjecture}

%Solution Environment
% \newenvironment{solution}
%               {\let\oldqedsymbol=\qedsymbol
%                 \renewcommand{\qedsymbol}{$\blacktriangleleft$}
%                 \begin{IEEEproof}[\bfseries\upshape Solution]}
%               {\end{IEEEproof}
%                 \renewcommand{\qedsymbol}{\oldqedsymbol}}
                
\newif\ifsolutions \solutionstrue

\def\preface
{
\chapter*{Preface}
\addcontentsline{toc}{chapter}{\protect
\numberline{Preface\string\hss}}
}

\newcommand{\mynote}[1]{\begin{center}
\fbox{\begin{minipage}{\columnwidth}{\begin{center} {\color{firebrick} \vspace{2mm} #1 \vspace{2mm}} \end{center}} \end{minipage}}\end{center}}



%%%%%%%%%% Mathematics Operators %%%%%%%%%
\DeclareMathOperator*{\Diag}{Diag}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\Tr}{Tr}
\DeclareMathOperator*{\cor}{cor}
\DeclareMathOperator*{\icr}{icr}
\DeclareMathOperator*{\lin}{lin}
\DeclareMathOperator*{\lina}{lina}
\DeclareMathOperator*{\relint}{relint}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\cconv}{cconv}
\DeclareMathOperator*{\ext}{ext}
\DeclareMathOperator*{\aff}{aff}
\DeclareMathOperator*{\codim}{codim}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\linspan}{span}
\DeclareMathOperator*{\lineal}{lineal}
\DeclareMathOperator*{\intt}{int}
\DeclareMathOperator*{\cone}{cone}
\DeclareMathOperator*{\qri}{qri}
\DeclareMathOperator*{\verts}{vert}

\newcommand{\primal}{\text{(CP)}}
\newcommand{\dual}[1]{\text{(D_{#1})}}
\newcommand{\oarrow}{\overset{\circ }{\rightarrow}}
\newcommand*{\dotcup}{\ensuremath{\mathaccent\cdot\cup}}
\newcommand*{\Proj}{\text{Proj}}
%\newcommand{\norm}[1]{\left\| {#1} \right\|}
\newcommand{\pwl}{\textrm{PWL}}
\newcommand{\poly}{\textrm{poly}}
\newcommand{\comp}{\textrm{comp}}
\newcommand{\brackets}[2][]{#1[#2 #1]}
\newcommand{\braces}[2][]{#1\{#2 #1\}}
%\newcommand{\set}[2][]{\braces[#1]{#2}}
\newcommand{\parens}[2][]{#1(#2 #1)}
\newcommand{\abs}[2][]{#1\lvert#2 #1\rvert}
\newcommand{\norm}[2][]{#1\lVert #2 #1\rVert}
\newcommand{\tuple}[2][]{#1 \langle #2 #1 \rangle}
\newcommand{\ip}[3][]{\tuple[#1]{#2,#3}}
% \Pr\parens{X = 0} or \Pr\parens[\Big]{X=0} to make parens }Big}
\DeclareMathOperator*{\relu}{{\textrm{ReLU}}}


%%%%%%%%%%%% Vectors %%%%%%%%%%%%%%
\def\ve#1{\mathchoice{\mbox{\boldmath$\displaystyle\bf#1$}}
{\mbox{\boldmath$\textstyle\bf#1$}}
{\mbox{\boldmath$\scriptstyle\bf#1$}}
{\mbox{\boldmath$\scriptscriptstyle\bf#1$}}}

%%%%%%%%%% Bold face letters  %%%%%%%%%%%%%
\newcommand{\rx}{{\ve r}}
\newcommand{\x}{{\ve x}}
\newcommand{\y}{{\ve y}}
\newcommand{\z}{{\ve z}}
% DOESNT WORK!? \renewcommand{\v}{{\ve v}}
% SO USE \ve{v} EXPLICITLY! 
\renewcommand{\v}{{\ve v}}
\newcommand{\g}{{\ve g}}
\newcommand{\e}{{\ve e}}
\renewcommand{\u}{{\ve u}}
\renewcommand{\a}{{\ve a}}
%\renewcommand{\b}{{\ve b}}
\renewcommand{\c}{{\ve c}}
\newcommand{\f}{{\ve f}}
\newcommand{\0}{{\ve 0}}
\newcommand{\m}{{\ve m}}
\newcommand{\p}{{\ve p}}
\renewcommand{\t}{{\ve t}}
\newcommand{\w}{{\ve w}}
\renewcommand{\b}{{\ve b}}
\renewcommand{\d}{{\ve d}}
\newcommand{\cve}{{\ve c}}
\newcommand{\h}{{\ve h}}
\newcommand{\q}{{\ve q}}
%\newcommand{\rve}{{\ve r}}
\newcommand{\var}[1]{\mathrm{var}\left( #1 \right)}
\newcommand{\I}{\textrm{I}}
\newcommand{\A}{\textrm{A}}
\newcommand{\B}{\textrm{B}}
\newcommand{\W}{\textrm{W}}
\newcommand{\C}{\textrm{C}}
\newcommand{\D}{\textrm{D}}
\newcommand{\U}{\textrm{U}}
\newcommand{\Rr}{\textrm{R}}
\newcommand{\s}{\textrm{s}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\FF}{\mathbb F}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\textrm{G}}
\newcommand{\bb}{\mathbb}
\newcommand{\R}{\bb R}
\newcommand{\Z}{{\bb Z}}
\newcommand{\N}{{\bb N}}
\newcommand{\Q}{{\bb Q}}
\newcommand{\cl}{\text{cl}}
\newcommand{\M}{\mathbf{M}}
\renewcommand{\C}{\mathcal C}
\renewcommand{\D}{\mathcal{D}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\ind}[1]{\mathds{1}_{\left\{#1\right\}}}
\newcommand\inlineeqno{\stepcounter{equation}\ (\theequation)}
\newcommand{\rnote}[1]{\textcolor{blue}{\textbf{[Ram: #1]}}}

%%%%%%%%%%%%%% END OF PREAMBLE %%%%%%%%%%%%%%%%%
